On cabled knots, Dehn surgery, and left-orderable fundamental groups

Previous work of the authors establishes a criterion on the fundamental group of a knot complement that determines when Dehn surgery on the knot will have a fundamental group that is not left-orderable. We provide a refinement of this criterion by introducing the notion of a decayed knot; it is shown that Dehn surgery on decayed knots produces surgery manifolds that have non-left-orderable fundamental group for all sufficiently positive surgeries. As an application, we prove that sufficiently positive cables of decayed knots are always decayed knots. These results mirror properties of L-space surgeries in the context of Heegaard Floer homology.

==> section/without-cases.tex <==
%without-cases.tex


We recall the construction of a cabled knot in order to fix notation. Consider the $(p,q)$-torus knot $T_{p,q}$, where $p, q >0$ are relatively prime. As the closure of a $p$-strand braid, this knot may be naturally viewed in a solid torus $T$ by removing a tubular neighbourhood of the braid axis. The complement of $T_{p,q}$ in $T$ is referred to as a $(p,q)$-cable space. Now given any knot $K$ in $S^3$, the cable knot $C_{p,q}(K)$ is obtained by identifying  the boundary of $T$ with the boundary of $S^3\smallsetminus\nu(K)$, identifying the longitude of $T$ with the longitude $\lambda$ of $K$. We will denote this cable knot by $C$ whenever this simplified notation does not cause confusion.

The knot group $\pi_1(C)$ may be calculate via the Seifert-Van Kampen Theorem, by viewing the complement $S^3\smallsetminus\nu(C)$ as the identification of the boundaries of $S^3\smallsetminus\nu(K)$ and a solid torus $D^2\times S^1$ along an essential annulus with core curve given by the slope $\mu^q\lambda^p$. If $\pi_1(D^2\times S^1)=\langle t \rangle$ then this gives rise to a natural amalgamated product
\[\pi_1(C)\cong\pi_1(K)\ast_{\mu^q\lambda^p=t^p}\bZ.\]

Consulting \cite[Section 3]{CW2010}, the meridian and longitude for $C$ may be calculated as \[\mC= \mu^u\lambda^vt^{-v} \quad {\rm and} \quad \lC= \mC^{-pq}t^p\] where $u$ and $v$ are positive integers satisfying $pu-qv=1$ (compare \cite[Proof of Theorem 3.1]{Tsau1988}). 

 \marginpar{I messed with this paragraph to make the transition. Alternatively, we could just  go for it and switch to $\sP$, etc. in the whole proof. The way we have set things up I don't know which is more natural. We do refer to positive elements constantly...}
Suppose that the knot $K$ is $r$-decayed, and choose cabling coefficients $p$ and $q$ so that $q/p >r$.  To begin, we choose a left-ordering of $\pi_1(C)$ and assume that $\mu_C^{pq} \lambda  = t^p\in\sP$.  This means that $t^p  = \mu^q \lambda^p\in\sP$, so every element $\mu^m \lambda^n$ is positive whenever $m/n >r$, since $K$ is $r$-decayed.  It will be convenient to make use of the fact that the existence of a positive cone is equivalent to a left-invariant strict total order by asserting that $g>1$ whenever $g\in\sP$  \cite{KME96}.

Our method of proof will be to check that the cable is $pq$-decayed by using the equivalence from Proposition \ref{prp:equiv}. In particular, we will show that for the given left-ordering $>$ of $\pi_1(C)$ with $\mu_C^{pq} \lambda_C >1$, there exists an unbounded sequence of increasing reduced rationals $\{r_i \}$ with $r_0 = pq$, such that $\alpha_{r_i} >1$ for all $i$.

First consider the case $\mu_C >1$. Here, $\mu_C^{pq+N} \lambda_C >1$ for $N \geq 0$,  as this is a product of positive elements. Therefore it suffices to choose $r_i = pq+i$ for all $i \geq 0$.

For the remainder of the proof, we assume that $\mu_C<1$.  For repeated use below, we also observe the crucial identity
\[ (t^{-v})^p (\mu^u \lambda^v)^p = (t^p)^{-v} \mu^{up} \lambda^{vp} = \mu^{-qv} \lambda^{-pv} \mu^{up} \lambda^{vp} = \mu^{pv -qu} = \mu,
\]
and recall that $t^p$ commutes with $\mu, \lambda, \mu_C$, and $\lambda_C$.   Therefore, we also have
\[ (\mu^u \lambda^v)^p (t^{-v})^p= (t^{-v})^p (\mu^u \lambda^v)^p  = \mu.
\]

Let $k$ be an arbitrary non-negative integer, and consider the element
\[ \mu^{-k} (t^{-v} \mu^u \lambda^v) \mu^k.
\] 
If this element is positive for some $k$, then the required sequence is provided by Lemma \ref{lem:lemma1} (proved below).  Therefore, we may assume that 
\[ \mu^{-k} (t^{-v} \mu^u \lambda^v) \mu^k <1
\]
for all $k$.

Similarly, for $k$ a non-negative integer, we consider
\[ (\mu^{-k} t^{-v} \mu^k)^{p-1} (\mu^u \lambda^v)^{p-1}.
\]
If this element is positive for some non-negative $k$, then we can create the required sequence using Lemma \ref{lem:lemma2} (proved below).
Therefore, we may assume that 
\[ (\mu^{-k} t^{-v} \mu^k)^{p-1} (\mu^u \lambda^v)^{p-1} <1
\]
for all $k$.

Observe that
\[ (\mu^{-k} t^{-v} \mu^k)^{p-1} (\mu^u \lambda^v)^{p-1}  = (\mu^{-k} t^{v} \mu^k) (\mu^{-k} t^{-vp} \mu^k)  (\mu^{up-u} \lambda^{vp-v}), 
\]
which, recalling that $t^p$ commutes with the elements $\mu$ and $\lambda$, simplifies to give
\[ (\mu^{-k} t^{v} \mu^k) (\mu^{-u} \lambda^{-v}) t^{-vp} \mu^{up} \lambda^{vp} =(\mu^{-k} t^{v} \mu^k) (\mu^{-u} \lambda^{-v}) \mu = \mu^{-k} t^{v} \lambda^{-v} \mu^{-u} \mu^{k+1} < 1 
\]
for all $k$. Taking inverses yields
\[ \mu^{-k-1} \mu^u \lambda^v t^{-v} \mu^k = \mu^{-k-1} \mu_C \mu^k >1,
\]
or $\mu_C \mu^k > \mu^{k+1}$ for all $k$.

Therefore taking $k=0$ we obtain $\mu_C > \mu$, so that left-multiplying by $\mu_C$ gives rise to
\[ \mu_C^2 > \mu_C \mu.
\]
When taking $k=1$, we get
\[\mu_C \mu > \mu^2,
\]
which combines with the previous expression to give $\mu_C^2 > \mu^2$.   Continuing in this manner, we obtain $\mu_C^N > \mu^N$ for all $N \geq 0$.

Left-multiplying by $t^p$, it follows that
\[ \mu_C^{N+pq} \lambda_C = \mu_C^N t^p > \mu^N t^p = \mu^{N+q} \lambda^p >1,
\]
where the final inequality follows from the fact that $(N+q)/p >q/p>r$ and $K$ is $r$-decayed.  As in the first case, we can choose our sequence of rationals to be $r_i = pq+i$ for all $i \geq 0$, and the theorem holds.

To conclude the proof, we establish Lemma \ref{lem:lemma1} and Lemma \ref{lem:lemma2}.

\begin{lemma}
\label{lem:lemma1}
If $\mu_C <1$ and $\mu^{-k} (t^{-v} \mu^u \lambda^v) \mu^k>1$ for some $k \geq 0$, then there exists a sequence of rationals $\{ r_i \}$ such that $\alpha_{r_i} >1$ for all $i$.
\end{lemma}
\begin{proof}
For $N \geq 0 $, we rewrite $\mu_C^N$ as
\[ \mu_C^N = \mu^u \lambda^v \mu^k (\mu^{-k} (t^{-v} \mu^u \lambda^v)^N \mu^k) \mu^{-u-k} \lambda^{-v}.
\]
Fix a positive integer $s$ that is large enough so that $(sq-u-k)/(sp-v) > r$, this is possible because $q/p>r$.   Next, the product $\mu_C^{N+pqs} \lambda_C^s = \mu_C^N t^{ps}$ becomes $\mu_C^N \mu^{sq} \lambda^{sp}$, which is equal to
\[ \mu^{u+k} \lambda^v (\mu^{-k} (t^{-v} \mu^u \lambda^v)^N \mu^k) (\mu^{qs-u-k} \lambda^{ps-v}).
\]
This is a product of positive elements, because:
\begin{enumerate}
\item $\mu^{u+k} \lambda^v >1$ because $(u+k)/v > q/p>r$, and 
\item $\mu^{qs-u-k} \lambda^{ps-v} >1$ because $(sq-u-k)/(sp-v) > r$,
\end{enumerate}
while the quantity $\mu^{-k} (t^{-v} \mu^u \lambda^v)^N \mu^k$ is positive by assumption.
Therefore, in this case we choose our sequence of rationals to be \[r_i = \frac{pqs+i}{s}\] for $i \geq 0$, this guarantees that the associated slopes $\alpha_{r_i}$ will be positive.  

%In the case that $\gcd( pqs+i, s ) =w >1$ observe that  $\alpha_{r_i}^w =\mu_C^{pqs+i} \lambda_C^s >1$, so that a positive power of $\alpha_{r_i}$ is positive.  

\end{proof}

\begin{lemma}
\label{lem:lemma2}
If $\mu_C <1$, $\mu^{-k} (t^{-v} \mu^u \lambda^v) \mu^k<1$ for all $k \geq 0$, and $ (\mu^{-k} t^{-v} \mu^k)^{p-1} (\mu^u \lambda^v)^{p-1} >1$ for some $k \geq 0$, then there exists a sequence of rationals $\{ r_i \}$ such that $\alpha_{r_i} >1$ for all $i$.
\end{lemma}
\begin{proof}
Fix $k \geq 0$ such that $\mu^{-k} (t^{-v} \mu^u \lambda^v) \mu^k<1$ and $ (\mu^{-k} t^{-v} \mu^k)^{p-1} (\mu^u \lambda^v)^{p-1} >1$, and
let $n$ be the smallest positive integer such that 
\[ (\mu^{-k} t^{-v} \mu^k)^{n} (\mu^u \lambda^v)^{n} >1,
\]
and
\[ (\mu^{-k} t^{-v} \mu^k)^{n-1} (\mu^u \lambda^v)^{n-1} <1,
\]
note that $1<n\leq q-1$.
Note that we may rearrange these two expressions, so that
\[ \mu^{-k} t^{-vn}  (\mu^u \lambda^v)^{n} \mu^k>1,
\]
and 
\[ \mu^{-k}  (\mu^u \lambda^v)^{1-n}  t^{-v(1-n)} \mu^k >1.
\] 
Then we can rewrite $\mu_C^N$ for $N \geq 1$ as follows:
\[ \mu_C^N = \mu^{u+k} \lambda^v (\mu^{-k} t^{-v(1-n)} \mu^k)[ (\mu^{-k} t^{-vn}  (\mu^u \lambda^v)^{n} \mu^k) \mu^{-k}  (\mu^u \lambda^v)^{1-n}  t^{-v(1-n)} \mu^k ]^{N-1} \mu^{-k} t^{-vn}.
\]
In the above expression, the quantity inside the square brackets is a product of positive elements.   Denote this quantity by P.  Choose an integer $s$ such that $(qs-k)/ps > r$.  Then considering the slope $\mu_C^{N+pq(v+s)} \lambda_C^{v+s} = \mu_C^N t^{p(v+s)}$, we find
\[ \mu_C^N t^{p(v+s)} = \mu^{u+k} \lambda^v (\mu^{-k} t^{-v(1-n)} \mu^k)P^{N-1} \mu^{qs-k}\lambda^{ps} t^{pv-vn} .
\]
This is a product of positive elements, because:
\begin{enumerate}
\item $\mu^{u+k} \lambda^v>1$, since $(u+k)/v > q/p > r$.
\item $\mu^{-k} t^{-v(1-n)}  \mu^k>1$, because if we consider its $p$-th power, we can use the fact that $t^p$ commutes with all peripheral elements so that
\[ (\mu^{-k} t^{-v(1-n)}  \mu^k)^p = t^{-pv(1-n)} >1.
\]
The final inequality follows from $-pv(1-n)>0$.
\item $\mu^{qs-k}\lambda^{ps} >1$, because $s$ is chosen so that $(qs-k)/ps > r$.  
\item $t^{pv-vn}>1$, because $pv-vn>0$.
\end{enumerate}
Therefore, in this case we may choose our sequence of rationals to be \[ r_i = \frac{i+pq(v+s)}{v+s} \] for $i \geq 0$, and $r_0 = pq$, as the corresponding slopes $\mu_C^{i+pq(v+s)} \lambda_C^{v+s} $ are positive in the left-ordering for $i \geq 0$.
\end{proof}

